Towards Generalizability to Tone and Content Variations in the Transcription of Amplifier Rendered Electric Guitar Audio

Transcribing electric guitar recordings is challenging due to the scarcity of diverse datasets and the complex tone-related variations introduced by amplifiers, cabinets, and effect pedals. To address these issues, we introduce EGDB-PG, a novel dataset designed to capture a wide range of tone-related characteristics across various amplifier-cabinet configurations. In addition, we propose the Tone-informed Transformer (TIT), a Transformer-based transcription model enhanced with a tone embedding mechanism that leverages learned representations to improve the model's adaptability to tone-related nuances. Experiments demonstrate that TIT, trained on EGDB-PG, outperforms existing baselines across diverse amplifier types, with transcription accuracy improvements driven by the dataset's diversity and the tone embedding technique. Through detailed benchmarking and ablation studies, we evaluate the impact of tone augmentation, content augmentation, audio normalization, and tone embedding on transcription performance. This work advances electric guitar transcription by overcoming limitations in dataset diversity and tone modeling, providing a robust foundation for future research.

==> tables/ablation.tex <==
\centering
\caption{Comprehensive evaluation of various settings, including tone removal, augmentations, and fine-tuning, in our model for low-gain, crunch, and high-gain transcription tasks on the EGDB v2 test-split. Baselines and comparisons with prior methods (e.g., MT3) are listed for reference.}
\label{tab:egdb_test}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc|cccccc|cccccc|cccccc}
\toprule
\textbf{Tone} & \textbf{Tone} & \textbf{GuitarSet v2} & \textbf{Norm} & \multicolumn{6}{c|}{\textbf{Low-gain}} & \multicolumn{6}{c|}{\textbf{Crunch}} & \multicolumn{6}{c}{\textbf{High-gain}} \\ 
\textbf{Removal}& \textbf{Emb.}& & & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c|}{Frame} & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c|}{Frame} & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c}{Frame} \\
& & & & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R \\
\midrule

% & & \checkmark & & 79.6 & \textbf{85.2} & 74.7 & 63.6 & 55.3 & 74.9 & 78.8 & 74.3 & 83.9 & 62.6 & 54.9 & 72.9 & 76.8 & 72.8 & 81.4 & 61.1 & 53.9 & 70.4 \\
 & \checkmark & \checkmark & & \textbf{84.0} & 81.5 & 86.6 & 68.4 & 59.4 & 80.1 & \textbf{81.6} & \textbf{77.6} & 86.0 & \textbf{67.6} & \textbf{58.7} & \textbf{79.8} & 78.9 & \textbf{75.5} & 82.6 & 64.5 & \textbf{56.5} & 75.3 \\
 \midrule
 & \checkmark & \checkmark & \checkmark & 83.2& 80.8 & 85.7 & \textbf{68.8} & \textbf{60.3} & \textbf{80.2} & 80.9 & 76.7 & 85.6 & 66.4 & 57.3 & 78.9 & \textbf{79.1} & 75.3 & 83.3 & \textbf{64.7} & 56.4 & \textbf{75.8} \\
 & DAC & \checkmark & & 79.5 & 77.9 & 81.2 & 63.2 & 56.3 & 71.9 & 79.4 & 79.7 & 79.1 & 62.8 & 56.5 & 70.7 &78.0 & 77.4 & 78.6 & 61.8 & 54.9 & 70.6 \\
 

& \checkmark& & & 58.4 & 73.4 & 48.5 & 46.6 & 47.1 & 53.8 & 60.3 & 64.1 & 57.0 & 48.4 & 42.1 & 56.8 & 54.6 & 58.8 & 50.9 & 44.8 & 38.5 & 53.5 \\
& \checkmark&  & \checkmark & 71.3 & 69.0 & 73.8 & 63.3 & 56.1 & 72.6 & 69.9 & 62.5 & 79.4 & 60.3 & 52.2 & 71.3 & 67.1 & 75.0 & 60.7 & 55.8 & 47.8 & 67.1 \\
\checkmark & \checkmark& & & 61.4 & 58.5 & 64.7 & 23.0 & 25.2 & 21.1 & 48.6 & 41.3 & 59.0 & 22.0 & 24.0 & 20.2 & 38.9 & 34.8 & 44.1 & 22.0 & 32.7 & 20.6 \\

\checkmark& \checkmark&  & \checkmark & 68.2 & 64.5 & 72.4 & 68.8 & 60.3 & 80.2 & 66.7 & 62.8 & 71.2 & 66.3 & 57.3 & 78.8 & 65.3 & 60.6 & 70.9 & 64.6 & 56.4 & 75.7 \\
% \midrule
% \multicolumn{22}{c}{\textbf{Baselines (hFT Transformer)}} \\
% \midrule


&&\checkmark&& 79.6 & \textbf{85.2} & 74.7 & 63.6 & 55.3 & 74.9 & 78.8 & 74.3 & 83.9 & 62.6 & 54.9 & 72.9 & 76.8 & 72.8 & 81.4 & 61.1 & 53.9 & 70.4 \\

\multicolumn{4}{c|}{hFT-Transformer baseline finetune EGDBv2} & 59.6 & 44.5 & \textbf{90.1} & 52.2 & 36.8 & \textbf{76.2} & 52.2 & 37.4 & 86.2 & 43.4 & 30.5 & 75.5 & 50.1 & 35.8 & 83.4 & 41.5 & 28.9 & 73.6 \\


\bottomrule
\end{tabular}%
  }


% \centering
% \caption{Comprehensive evaluation of various settings, including tone removal, augmentations, and fine-tuning, in our model for low-gain, crunch, and high-gain transcription tasks on the EGDB v2 test-split. Baselines and comparisons with prior methods (e.g., MT3) are listed for reference.}
% \label{tab:egdb_test}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{cccc|ccc|ccc|ccc}
% \toprule
% \textbf{Tone} & \textbf{Tone} & \textbf{GuitarSet v2} & \textbf{Norm} & \multicolumn{3}{c|}{\textbf{Low-gain}} & \multicolumn{3}{c|}{\textbf{Crunch}} & \multicolumn{3}{c}{\textbf{High-gain}} \\ 
% \textbf{Removal} & \textbf{Emb.} & & & \multicolumn{1}{c}{Onset} & \multicolumn{1}{c}{Frame} & & \multicolumn{1}{c}{Onset} & \multicolumn{1}{c}{Frame} & & \multicolumn{1}{c}{Onset} & \multicolumn{1}{c}{Frame} & \\

% & & & & F1 & F1 & & F1 & F1 & & F1 & F1 & \\
% \midrule

%  & \checkmark & \checkmark & & \textbf{84.0} & 68.4 & & \textbf{81.6} & \textbf{67.6} & & 78.9 & 64.5 & \\
%  \midrule
%  & \checkmark & \checkmark & \checkmark & 83.2 & \textbf{68.8} & & 80.9 & 66.4 & & \textbf{79.1} & \textbf{64.7} & \\
%  & DAC & \checkmark & & 79.5 & 63.2 & & 79.4 & 62.8 & & 78.0 & 61.8 & \\
%  & \checkmark & & & 58.4 & 46.6 & & 60.3 & 48.4 & & 54.6 & 44.8 & \\
%  & \checkmark & & \checkmark & 71.3 & 63.3 & & 69.9 & 60.3 & & 67.1 & 55.8 & \\
%  \checkmark & \checkmark & & & 61.4 & 23.0 & & 48.6 & 22.0 & & 38.9 & 22.0 & \\
%  \checkmark & \checkmark & & \checkmark & 68.2 & 68.8 & & 66.7 & 66.3 & & 65.3 & 64.6 & \\
%  && \checkmark & & 79.6 & 63.6 & & 78.8 & 62.6 & & 76.8 & 61.1 & \\

% \multicolumn{4}{c|}{hFT-Transformer baseline finetune EGDBv2} & 59.6 & 52.2 & & 52.2 & 43.4 & & 50.1 & 41.5 & \\

% \bottomrule
% \end{tabular}%
% }


==> tables/icassp_comparison.tex <==
% \centering
% \caption{Evaluation of various settings, including tone removal, augmentations, and fine-tuning, in our model for low-gain, crunch, and high-gain transcription tasks on the 4th and 5th amps in EGDB v1.}
% \label{tab:egdb_test_ICASSP}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccc|cccccc|}
% \toprule
% \textbf{Tone} & \textbf{Tone} & \textbf{GuitarSet v2} & \textbf{Norm} & \multicolumn{6}{c|}{\textbf{4th,5th amps in EGDBv1}} \\ 
% \textbf{Removal}& \textbf{Emb.}& \textbf{Aug.}& & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c|}{Frame}\\
% & & & & F1 & P & R & F1 & P & R  \\
% \midrule
% \multicolumn{10}{c}{\textbf{Our Model}} \\

% \midrule
% % & & \checkmark & & 79.6 & \textbf{85.2} & 74.7 & 63.6 & 55.3 & 74.9 & 78.8 & 74.3 & 83.9 & 62.6 & 54.9 & 72.9 & 76.8 & 72.8 & 81.4 & 61.1 & 53.9 & 70.4 \\
%  & \checkmark & \checkmark & & \textbf{85.1} & \textbf{84.3} & 86.0 & \textbf{70.8} & \textbf{62.7} & \textbf{81.3}  \\
%  & \checkmark & \checkmark & \checkmark & 83.1 & 80.3 & \textbf{86.2} & 68.7 & 59.6 & 81.1  \\
 
% % \midrule
% % \multicolumn{10}{c}{\textbf{Additional Ablations}} \\
% % \midrule
% & \checkmark& & & 53.9 & 76.7 & 41.5 & 41.7 & 38.1 & 46.0  \\
% & \checkmark&  & \checkmark & 70.9 & 64.8 & 78.4 & 61.8 & 53.7 & 72.8  \\
% \midrule

% \multicolumn{10}{c}{\textbf{Baselines}} \\
% \midrule
% \multicolumn{4}{c|}{hFT-Transformer \cite{toyama2023automatic}}  & 81.9 & 78.6 & 85.5 & 67.6 & 58.5 & 80.2 \\
% \multicolumn{4}{c|}{Seq2Seq\cite{chen2022towards}}   & 59.2 & n/a & n/a & 52.6 & n/a & n/a\\
% \bottomrule
% \end{tabular}%
%   }

  
\centering
\caption{Evaluation of tone embeddings, GuitarSetv2 augmentation, and audio normalization in our tone embedding-informed hFT-Transformer model assesses transcription performance on unseen amplifier tones (JC120 and Marshall) in EGDBv1, compared to Seq2Seq and hFT-Transformer baselines.}
\label{tab:egdb_test_ICASSP}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc|cccccc|}
\toprule
\textbf{GuitarSet v2} & \textbf{Norm} & \multicolumn{6}{c|}{\textbf{4th,5th amps in EGDBv1}} \\ 
\textbf{Aug.}& & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c|}{Frame}\\
& & F1 & P & R & F1 & P & R  \\
\midrule
\multicolumn{8}{c}{\textbf{Ourmodel (Tone informed hFT-Transformer)}} \\

\midrule
\checkmark & & \textbf{85.1} & \textbf{84.3} & 86.0 & \textbf{70.8} & \textbf{62.7} & \textbf{81.3}  \\
\checkmark & \checkmark & 83.1 & 80.3 & \textbf{86.2} & 68.7 & 59.6 & 81.1  \\
 
& & 53.9 & 76.7 & 41.5 & 41.7 & 38.1 & 46.0  \\
& \checkmark & 70.9 & 64.8 & 78.4 & 61.8 & 53.7 & 72.8  \\

\midrule
\multicolumn{8}{c}{\textbf{Baselines}} \\
\midrule

\multicolumn{2}{l|}{hFT-Transformer \cite{toyama2023automatic}}  & 81.9 & 78.6 & 85.5 & 67.6 & 58.5 & 80.2 \\
\multicolumn{2}{l|}{Seq2Seq\cite{chen2022towards}}   & 59.2 & n/a & n/a & 52.6 & n/a & n/a\\
\bottomrule
\end{tabular}%
}

% double column version
% \centering
% \caption{Evaluation of various settings, including tone embeddings, GuitarSetv2 augmentation, and audio normalization, in our tone embedding-informed hFT-Transformer model for low-gain, crunch, and high-gain transcription tasks on the fourth and fifth amplifiers (JC120 and Marshall) in EGDBv1, compared to baselines, assesses performance on unseen amplifier tones. Our model with tone embeddings and GuitarSetv2 augmentation outperforms both baselines: Seq2Seq from \cite{chen2022towards} and hFT-Transformer from \cite{toyama2023automatic}. Audio normalization improves performance in low-resource conditions, enhancing stability when training data diversity is limited, but its benefits decrease when GuitarSetv2 augmentation is applied, as the model adapts to the increased content diversity. These results also highlight GuitarSetv2’s critical role in improving accuracy for unseen amplifier tones in EGDB.}
% \label{tab:egdb_test_ICASSP}
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{12pt} % Adjust column spacing
% \resizebox{0.85\textwidth}{!}{ % Adjust table width
% \begin{tabular}{cc|cccccc|}
% \toprule
% \textbf{GuitarSet v2} & \textbf{Norm} & \multicolumn{6}{c|}{\textbf{4th,5th amps in EGDBv1}} \\ 
% \textbf{Aug.} & & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c|}{Frame}\\
% & & F1 & P & R & F1 & P & R  \\
% \midrule
% \multicolumn{8}{c}{\textbf{Our Model (Tone Embedding Informed hFT-Transformer)}} \\
% \midrule
% \checkmark & & \textbf{85.1} & \textbf{84.3} & 86.0 & \textbf{70.8} & \textbf{62.7} & \textbf{81.3}  \\
% \checkmark & \checkmark & 83.1 & 80.3 & \textbf{86.2} & 68.7 & 59.6 & 81.1  \\
% & & 53.9 & 76.7 & 41.5 & 41.7 & 38.1 & 46.0  \\
% & \checkmark & 70.9 & 64.8 & 78.4 & 61.8 & 53.7 & 72.8  \\
% \midrule
% \multicolumn{8}{c}{\textbf{Baselines}} \\
% \midrule
% \multicolumn{2}{c|}{hFT-Transformer \cite{toyama2023automatic}}  & 81.9 & 78.6 & 85.5 & 67.6 & 58.5 & 80.2 \\
% \multicolumn{2}{c|}{Seq2Seq \cite{chen2022towards}}   & 59.2 & n/a & n/a & 52.6 & n/a & n/a\\
% \bottomrule
% \end{tabular}%
% }


==> tables/original_table_1.tex <==
\centering
\caption{Comprehensive evaluation of various settings, including tone removal, augmentations, and fine-tuning, in our model for low-gain, crunch, and high-gain transcription tasks on the EGDB v2 test-split. Baselines and comparisons with prior methods (e.g., MT3) are listed for reference.}
\label{tab:egdb_test}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc|cccccc|cccccc|cccccc}
\toprule
\textbf{Tone} & \textbf{Tone} & \textbf{GuitarSet v2} & \textbf{Norm} & \multicolumn{6}{c|}{\textbf{Low-gain}} & \multicolumn{6}{c|}{\textbf{Crunch}} & \multicolumn{6}{c}{\textbf{High-gain}} \\ 
\textbf{Removal}& \textbf{Emb.}& \textbf{Aug.}& & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c|}{Frame} & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c|}{Frame} & \multicolumn{3}{c}{Onset} & \multicolumn{3}{c}{Frame} \\
& & & & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R \\
\midrule
\multicolumn{22}{c}{\textbf{Our Model}} \\

\midrule
% & & \checkmark & & 79.6 & \textbf{85.2} & 74.7 & 63.6 & 55.3 & 74.9 & 78.8 & 74.3 & 83.9 & 62.6 & 54.9 & 72.9 & 76.8 & 72.8 & 81.4 & 61.1 & 53.9 & 70.4 \\
 & \checkmark & \checkmark & & \textbf{84.0} & 81.5 & 86.6 & 68.4 & 59.4 & 80.1 & \textbf{81.6} & \textbf{77.6} & 86.0 & \textbf{67.6} & \textbf{58.7} & \textbf{79.8} & 78.9 & \textbf{75.5} & 82.6 & 64.5 & \textbf{56.5} & 75.3 \\
 & DAC & \checkmark & & 79.5 & 77.9 & 81.2 & 63.2 & 56.3 & 71.9 & 79.4 & 79.7 & 79.1 & 62.8 & 56.5 & 70.7 &78.0 & 77.4 & 78.6 & 61.8 & 54.9 & 70.6 \\
 & \checkmark & \checkmark & \checkmark & 83.2& 80.8 & 85.7 & \textbf{68.8} & \textbf{60.3} & \textbf{80.2} & 80.9 & 76.7 & 85.6 & 66.4 & 57.3 & 78.9 & \textbf{79.1} & 75.3 & 83.3 & \textbf{64.7} & 56.4 & \textbf{75.8} \\
 
\midrule
\multicolumn{22}{c}{\textbf{Our Model without augmentation}} \\
\midrule
& \checkmark& & & 58.4 & 73.4 & 48.5 & 46.6 & 47.1 & 53.8 & 60.3 & 64.1 & 57.0 & 48.4 & 42.1 & 56.8 & 54.6 & 58.8 & 50.9 & 44.8 & 38.5 & 53.5 \\
& \checkmark&  & \checkmark & 71.3 & 69.0 & 73.8 & 63.3 & 56.1 & 72.6 & 69.9 & 62.5 & 79.4 & 60.3 & 52.2 & 71.3 & 67.1 & 75.0 & 60.7 & 55.8 & 47.8 & 67.1 \\
\checkmark & \checkmark& & & 61.4 & 58.5 & 64.7 & 23.0 & 25.2 & 21.1 & 48.6 & 41.3 & 59.0 & 22.0 & 24.0 & 20.2 & 38.9 & 34.8 & 44.1 & 22.0 & 32.7 & 20.6 \\

\checkmark& \checkmark&  & \checkmark & 68.2 & 64.5 & 72.4 & 68.8 & 60.3 & 80.2 & 66.7 & 62.8 & 71.2 & 66.3 & 57.3 & 78.8 & 65.3 & 60.6 & 70.9 & 64.6 & 56.4 & 75.7 \\
\midrule
\multicolumn{22}{c}{\textbf{Baselines (hFT Transformer)}} \\
\midrule


\multicolumn{4}{c|}{EGDB v2 and GuitarSet v2} & 79.6 & \textbf{85.2} & 74.7 & 63.6 & 55.3 & 74.9 & 78.8 & 74.3 & 83.9 & 62.6 & 54.9 & 72.9 & 76.8 & 72.8 & 81.4 & 61.1 & 53.9 & 70.4 \\
\multicolumn{4}{c|}{Maestro} & 74.4 & 64.3 & 88.5 & 54.5 & 47.1 & 64.6 & 47.5 & 32.4 & \textbf{89.2} & 42.2 & 32.0 & 61.9 & 42.6 & 28.3 & \textbf{86.4} & 39.1 & 29.4 & 58.4 \\
\multicolumn{4}{c|}{finetune EGDB v2} & 59.6 & 44.5 & \textbf{90.1} & 52.2 & 36.8 & \textbf{76.2} & 52.2 & 37.4 & 86.2 & 43.4 & 30.5 & 75.5 & 50.1 & 35.8 & 83.4 & 41.5 & 28.9 & 73.6 \\
\midrule

\multicolumn{22}{c}{\textbf{Baselines (MT3)}} \\
\midrule
\multicolumn{4}{c|}{MT3 - Guitar} & 44.2 & 34.7 & 60.7 & 7.9 & 12.8 & 5.7 & 50.6 & 40.9 & 66.2 & 9.9 & 13.7 & 7.7 & 46.8 & 38.5 & 59.8 & 7.8 & 9.7 & 6.5 \\
\multicolumn{4}{c|}{MT3 - Guitar \& Piano} & 73.5 & 65.9 & 83.2 & 9.8 & 9.9 & 9.8 & 73.3 & 68.6 & 78.7 & 12.7 & 11.8 & 13.7 & 70.0 & 65.5 & 75.2 & 10.0 & 9.1 & 11.1 \\

\bottomrule
\end{tabular}%
  }

